Optimal Bidding Strategies for Online Ad Auctions with Overlapping Targeting Criteria

We analyze the problem of how to optimally bid for ad spaces in online ad auctions. For this we consider the general case of multiple ad campaigns with overlapping targeting criteria. In our analysis we first characterize the structure of an optimal bidding strategy. In particular, we show that an optimal bidding strategies decomposes the problem into disjoint sets of campaigns and targeting groups. In addition, we show that pure bidding strategies that use only a single bid value for each campaign are not optimal when the supply curves are not continuous. For this case, we derive a lower-bound on the optimal cost of any bidding strategy, as well as mixed bidding strategies that either achieve the lower-bound, or can get arbitrarily close to it.

==> intuition.tex <==

\section{Intuition}\label{sec:intuition}

Before we start with the analysis, we consider the special case where we are have a single campaign $i=1$ and a single targeting group $j=1$. This is the simplest non-trivial case will provide insight into the structure of an optimal bidding strategy.

We first consider this case under the assumption that the supply curve for the targeting group is continuous. For this case, the optimal strategy is to bid for all impression, i.e. we have that
$$\gamma_{1,1} = 1$$
with bid value $b_{1,1}$ such that
$$ D_1(b_{1,1}) = I_1.$$

Next we consider the case where the supply curve $D_1(b)$ has to steps where
$$ D_1(b_1) < I_1 < D_1(b_2).$$
If campaign is able to bid with only one value $b_{1,1}$, then the optimal bid allocation is to bid value
$$b_{1,1} = b_2$$
with
$$\gamma_{1,1} = \frac{I_1}{ D_1(b_2)}.$$
The resulting cost is
$$ \gamma_{1,1} [ b_1 D_1(b_1) + b_2 ( D_1(b_2) -  D_1(b_2))] < [ b_1 D_1(b_1) + b_2 ( D_1(b_2) -  D_1(b_2))].$$

